One Body, Two Minds: Alternating VR Perspective During Remote Teleoperation of Supernumerary Limbs

Remote VR teleoperation with supernumerary robotic limbs enables distant users to operate in another's local space. While a shared first-person view aids hand-eye coordination, locking the guest's camera to the host's head can degrade comfort, embodiment, and coordination. Based on a formative study (N=10) using a virtual supernumerary robotic limbs configuration to stress-test coordination, we propose guest-driven perspective switching from a shared first-person baseline (Shared Embodied View) to two alternatives: (a) a stabilized view with guest-controlled rotation (Embedded Anchored View), and (b) a fully decoupled third-person view (Out-of-body View). We ran a user study with 24 pairs (N=48) who switched between the baseline and proposed views as task demands changed. We measured performance, embodiment, fatigue, physiological arousal, and switching behaviors. Our results reveal role-dependent trade-offs: Out-of-body View improves navigation efficiency and reduces errors, while Embedded Anchored View supports embodiment. We conclude with guidelines: use Embedded Anchored View for hand-centric adjustments, Out-of-body View for navigation and object placement, and ensure smooth transitions.

==> sections/glmm_model_specification.tex <==
% !TEX root = ../Sharedperspective.tex

\noindent\textbf{Embodiment Score GLMM:}
\begin{equation}
\begin{aligned}
\text{EmbodimentScore}_{ijkl} &= \beta_0 
+ \beta_1(\text{Perspective}_i) 
+ \beta_2(\text{UserRole}_j) \\
&\quad + \beta_3(\text{Factor}_k) 
+ \beta_4(\text{Perspective}_i \times \text{UserRole}_j) \\
&\quad + \beta_5(\text{Perspective}_i \times \text{Factor}_k) 
+ u_l + \epsilon_{ijkl}, \\
u_l &\sim \mathcal{N}(0, \sigma_u^2), \quad 
\epsilon_{ijkl} \sim \mathcal{N}(0, \sigma_\epsilon^2)
\end{aligned}
\end{equation}

\noindent\textbf{VAS-F (Fatigue) GLMM:}
\begin{equation}
\small
\begin{aligned}
\log(\text{VAS-F}_{ijk}) &=\beta_0 + \beta_1(\text{Perspective}_i) + \beta_2(\text{Task}_k) + \beta_3(\text{UserRole}_j) \\
&\quad+ \beta_4(\text{Perspective}_i \times \text{UserRole}_j) + \beta_5(\text{Perspective}_i \times \text{Task}_k) \\
&\quad+ u_i + \epsilon_{ijk},\\
u_i &\sim \mathcal{N}(0, \sigma_u^2), \quad \epsilon_{ijk} \sim \mathcal{N}(0, \sigma_\epsilon^2)
\end{aligned}
\end{equation}

\noindent\textbf{NASA-TLX (Workload) GLMM:}
\begin{equation}
\small
\begin{aligned}
\text{NASA-TLX}_{ijk} &=\beta_0 + \beta_1(\text{Perspective}_i) + \beta_2(\text{Task}_k) + \beta_3(\text{UserRole}_j) \\
&\quad+ \beta_4(\text{Perspective}_i \times \text{UserRole}_j) + \beta_5(\text{Perspective}_i \times \text{Task}_k) \\
&\quad+ u_i + \epsilon_{ijk},\\
u_i &\sim \mathcal{N}(0, \sigma_u^2), \quad \epsilon_{ijk} \sim \mathcal{N}(0, \sigma_\epsilon^2)
\end{aligned}
\end{equation}

\noindent\textbf{Task Performance GLMM:}
\begin{equation}
\small
\begin{split}
\log(\text{Performance}_{ijk}) &=\beta_0 + \beta_1(\text{Perspective}_i) + \beta_2(\text{Task}_j) \\
&+ \beta_3(\text{Perspective}_i \times \text{Task}_j) + u_k + \epsilon_{ijk}, \\
u_k &\sim \mathcal{N}(0,\sigma^2_u),\quad \epsilon_{ijk}\sim\mathcal{N}(0,\sigma^2_{\epsilon})
\end{split}
\end{equation}

\noindent\textbf{Perspective Switching GLMM:}
\begin{equation}
\small
\begin{split}
\log(\text{SwitchCount}_{ijkl}) &=\beta_0 + \beta_1(\text{Perspective}_i) + \beta_2(\text{TaskPhase}_j) \\
&\quad + \beta_3(\text{UserRole}_k) + \beta_4(\text{Perspective}_i \times \text{TaskPhase}_j) \\
&\quad + u_l + \epsilon_{ijkl}, \\
u_l &\sim \mathcal{N}(0,\sigma^2_u), \quad \epsilon_{ijkl}\sim\mathcal{N}(0,\sigma^2_{\epsilon})
\end{split}
\end{equation}

\noindent\textbf{Heart Rate (HRV) GLMM:}
\begin{equation}
\small
\begin{split}
\text{HRV}_{ijkl} &=\beta_0 + \beta_1(\text{Perspective}_i) + \beta_2(\text{UserRole}_j) + \beta_3(\text{Measure}_k) \\
&\quad + \beta_4(\text{Perspective}_i \times \text{UserRole}_j) + u_l + \epsilon_{ijkl}, \\
u_l &\sim \mathcal{N}(0,\sigma^2_u), \quad \epsilon_{ijkl}\sim\mathcal{N}(0,\sigma^2_{\epsilon})
\end{split}
\end{equation}


==> sections/table/embodiment_glmm.tex <==
%!TEX root = ../Sharedperspective.tex

\begin{table}[htbp]
\centering
\caption{Generalized Linear Mixed Model (GLMM) results for Embodiment Scores}
\label{tab:embodiment_glmm}
\small
\begin{tabular}{lccc}
\toprule
\textbf{Contrast (Role, Factor)} & \textbf{Estimate} & \textbf{SE} & \textbf{p-value} \\
\midrule
\textit{Agency (HU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.500 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & 0.667 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & 0.167 & 0.111 & 0.293 \\
\midrule
\textit{Agency (GU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.875 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & -0.583 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & -1.458 & 0.111 & \textbf{<0.0001} \\
\midrule
\textit{Body Ownership (HU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.667 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & 0.813 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & 0.146 & 0.111 & 0.391 \\
\midrule
\textit{Body Ownership (RU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.646 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & -0.708 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & -1.354 & 0.111 & \textbf{<0.0001} \\
\midrule
\textit{Presence/Identification (HU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.542 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & 0.917 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & 0.375 & 0.111 & \textbf{0.0023} \\
\midrule
\textit{Presence/Identification (GU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.521 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & -0.875 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & -1.396 & 0.111 & \textbf{<0.0001} \\
\midrule
\textit{Sensory Integration/Self-location (HU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.563 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & 0.604 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & 0.042 & 0.111 & 0.926 \\
\midrule
\textit{Sensory Integration/Self-location (GU)} & & & \\
Embedded Anchored vs. Out-of-body & 0.875 & 0.111 & \textbf{<0.0001} \\
Embedded Anchored vs. Shared Embodied & -0.563 & 0.111 & \textbf{<0.0001} \\
Out-of-body vs. Shared Embodied & -1.438 & 0.111 & \textbf{<0.0001} \\
\bottomrule
\multicolumn{4}{p{8.5cm}}{\scriptsize Note: Significant effects (p < .05) highlighted in bold.}\end{tabular}
\end{table}

==> sections/table/glmm_WF.tex <==
%!TEX root = ../Sharedperspective.tex

\begin{table}[htbp]
\centering
\caption{GLMM Results for Perspective Switching Frequency}
\label{tab:GLMM-switching}
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{p{4cm}ccc}
\toprule
\textbf{Variable} & \textbf{Estimate} & \textbf{Std. Error} & \textbf{p-value} \\
\midrule
\multicolumn{4}{l}{\textbf{Main Effects}} \\
Perspective = \textit{Out-of-body View} & 1.24 & 0.36 & 0.001 \\
Perspective = \textit{Embedded Anchored View} & 1.96 & 0.38 & \textbf{<0.001} \\
User Role = GU & 0.78 & 0.27 & 0.004 \\
Task Phase = Navigation & 1.35 & 0.33 & \textbf{<0.001} \\
Task Phase = Visual Search & 0.67 & 0.30 & 0.028 \\
\midrule
\multicolumn{4}{l}{\textbf{Interaction Effects}} \\
\textit{Out-of-body View} : GU & 0.56 & 0.31 & 0.070 \\
\textit{Embedded Anchored View} : GU & 0.72 & 0.32 & 0.024 \\
\textit{Out-of-body View} : Navigation & 1.10 & 0.34 & 0.001 \\
\textit{Embedded Anchored View} : Navigation & -0.42 & 0.36 & 0.231 \\
\textit{Out-of-body View} : Visual Search & -0.35 & 0.33 & 0.290 \\
\textit{Embedded Anchored View} : Visual Search & 0.24 & 0.35 & 0.490 \\
\bottomrule
\multicolumn{4}{p{8.2cm}}{\scriptsize Note: Baseline = \textit{Shared Embodied View}; User Role baseline = HU; Task Phase baseline = Precision. Significant effects are highlighted in bold.}
\end{tabular}
\end{table}


==> sections/table/glmm_heartrate.tex <==
%!TEX root = ../Sharedperspective.tex

\begin{table}[htbp]
\centering
\caption{GLMM Results for Subjective Fatigue (VAS-F) and Workload (NASA-TLX)}
\label{tab:glmm-WF}
\small
\begin{tabular}{p{4.1cm}ccc}
\toprule
\textbf{Variable} & \textbf{Estimate} & \textbf{Std. Error} & \textbf{p-value} \\
\midrule
\multicolumn{4}{l}{\textbf{VAS-F (Fatigue)}} \\
Intercept & 3.24 & 0.15 & \textbf{<0.001} \\
Perspective (\textit{Embedded Anchored View} vs. \textit{Out-of-body View}) & 0.36 & 0.11 & 0.001 \\
Task (Transportation vs. Factory) & 0.12 & 0.10 & 0.226 \\
User Role (GU vs. HU) & 0.45 & 0.13 & 0.001 \\
Perspective × User Role & 0.42 & 0.14 & 0.003 \\
Perspective × Task & 0.09 & 0.12 & 0.452 \\
\midrule
\multicolumn{4}{l}{\textbf{NASA-TLX (Workload)}} \\
Intercept & 46.20 & 1.40 & \textbf{<0.001} \\
Perspective (\textit{Embedded Anchored View} vs. \textit{Out-of-body View}) & 1.20 & 1.02 & 0.238 \\
Task (Transportation vs. Factory) & -1.34 & 1.11 & 0.229 \\
User Role (GU vs. HU) & 0.92 & 1.08 & 0.393 \\
Perspective × User Role & 3.42 & 1.14 & 0.003 \\
Perspective × Task & 2.86 & 1.06 & 0.007 \\
\bottomrule
\multicolumn{4}{p{8.2cm}}{\scriptsize Note: Perspective baseline = \textit{Out-of-body View}; Task baseline = Factory; User Role baseline = HU. Significant effects highlighted in bold.}
\end{tabular}
\end{table}

==> sections/table/glmm_performance.tex <==
%!TEX root = ../Sharedperspective.tex

\begin{table}[htbp]
\centering
\caption{GLMM Results for Task Performance (Completion Time and Error Rate)}
\label{tab:glmm-performance}
\small
\begin{tabular}{p{4cm}ccc}
\toprule
\textbf{Variable} & \textbf{Estimate} & \textbf{Std. Error} & \textbf{p-value} \\
\midrule
\multicolumn{4}{l}{\textbf{Completion Time}} \\
Intercept & 1.78 & 0.08 & \textbf{<0.001} \\
Perspective (out-of-body view vs. embedded anchored view) & -0.28 & 0.09 & 0.002 \\
Task (Transportation vs. Factory) & 0.19 & 0.10 & 0.060 \\
Perspective × Task & 0.34 & 0.11 & 0.002 \\
\midrule
\multicolumn{4}{l}{\textbf{Error Rate}} \\
Intercept & 1.53 & 0.07 & \textbf{<0.001} \\
Perspective (out-of-body view vs. embedded anchored view) & -0.41 & 0.12 & \textbf{<0.001} \\
Task (Transportation vs. Factory) & -0.15 & 0.11 & 0.173 \\
Perspective × Task & 0.38 & 0.14 & 0.007 \\
\bottomrule
\multicolumn{4}{p{8.2cm}}{\scriptsize Note: Perspective baseline = Embedded Anchored View; Task baseline = Factory. Significant effects highlighted in bold.}
\end{tabular}
\end{table}

==> sections/table/glmm_switching.tex <==
%!TEX root = ../Sharedperspective.tex

\begin{table}[htbp]
\centering
\caption{GLMM Results for Perspective Switching Frequency}
\label{tab:GLMM-switching}
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\linewidth}{l>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
\toprule
\textbf{Variable} & \textbf{Estimate} & \textbf{Std. Error} & \textbf{p-value} \\
\midrule
\multicolumn{4}{l}{\textbf{Main Effects}} \\
Perspective = \textit{Out-of-body View} & 1.24 & 0.36 & 0.001 \\
Perspective = \textit{Embedded Anchored View} & 1.96 & 0.38 & \textbf{<0.001} \\
User Role = GU & 0.78 & 0.27 & 0.004 \\
Task Phase = Navigation & 1.35 & 0.33 & \textbf{<0.001} \\
Task Phase = Visual Search & 0.67 & 0.30 & 0.028 \\
\midrule
\multicolumn{4}{l}{\textbf{Interaction Effects}} \\
\textit{Out-of-body View} : GU & 0.56 & 0.31 & 0.070 \\
\textit{Embedded Anchored View} : GU & 0.72 & 0.32 & 0.024 \\
\textit{Out-of-body View} : Navigation & 1.10 & 0.34 & 0.001 \\
\textit{Embedded Anchored View} : Navigation & -0.42 & 0.36 & 0.231 \\
\textit{Out-of-body View} : Visual Search & -0.35 & 0.33 & 0.290 \\
\textit{Embedded Anchored View} : Visual Search & 0.24 & 0.35 & 0.490 \\
\bottomrule
\multicolumn{4}{p{0.97\linewidth}}{\scriptsize Note: Baseline = \textit{Shared Embodied View}; User Role baseline = HU; Task Phase baseline = Precision. Significant effects are highlighted in bold.}
\end{tabularx}
\end{table}

